Measuring Personalization of Web Search

Web search is an integral part of our daily lives. Recently, there has been a trend of personalization in Web search, where different users receive different results for the same search query. The increasing level of personalization is leading to concerns about Filter Bubble effects, where certain users are simply unable to access information that the search engines' algorithm decides is irrelevant. Despite these concerns, there has been little quantification of the extent of personalization in Web search today, or the user attributes that cause it. In light of this situation, we make three contributions. First, we develop a methodology for measuring personalization in Web search results. While conceptually simple, there are numerous details that our methodology must handle in order to accurately attribute differences in search results to personalization. Second, we apply our methodology to 200 users on Google Web Search and 100 users on Bing. We find that, on average, 11.7% of results show differences due to personalization on Google, while 15.8% of results are personalized on Bing, but that this varies widely by search query and by result ranking. Third, we investigate the user features used to personalize on Google Web Search and Bing. Surprisingly, we only find measurable personalization as a result of searching with a logged in account and the IP address of the searching user. Our results are a first step towards understanding the extent and effects of personalization on Web search engines today.

==> acknowledgements.tex <==
\section*{Acknowledgements}

We thank the anonymous reviewers for their helpful comments. 
This research was supported by NSF grants IIS-0964465 and CNS-1054233, and an Amazon Web Services in Education Grant.


==> related.tex <==
\section{Related Work}
\label{sec:related}

%~\cite{kendall-1938-tau}

%\paragraph{Comparing Search Results and Engines} Comparing ranked lists, such as search engine
%results, is an active topic in the Information Retrieval (IR) community. Several studies
%improve the classic Kendall's $\tau$ metric by adding per-rank
%weights~\cite{fagin-2003-topk,shieh-2000-independence}, and by taking item similarity into
%account~\cite{sculley-2007-rankaggregation,kumar-2010-rankings}. DCG and NDCG use a logarithmic scale
%to reduce the scores of bottom ranked items~\cite{jarvelin-2000-evaluation}. The cascade
%model~\cite{craswell-2007-clickposition} and its successor ERR~\cite{chapelle-2009-rank} extend DCG
%by taking the relatedness of subsequent list items into account. Two recent studies develop
%probabilistic metrics that penalizing errors at top ranks without requiring explicit
%weights~\cite{yilmaz-2008-newrank,carterette-2009-rankcorrelation}.

%Classical metrics
%such as Spearman's footrule and $\rho$~\cite{spearman-1904-association,diaconis-1977-disarray} and Kendall's
%$\tau$~\cite{kendall-1938-tau} both calculate pairwise disagreements between ordered lists.
%However, these classic metrics do not take into account that when evaluating results
%from search engines, disagreements among low ranking items (\eg rank 1) are more costly.
%Numerous new metrics have been proposed to address this shortcoming.
%Fagin \etal~\cite{fagin-2003-topk} and Shieh \etal~\cite{weighted_kt-00}
%both propose modifications of Kendall's $\tau$ that incorporate per-rank weights.
%Discounted Cumulative Gain (DCG) and Normalized Discounted Cumulative Gain (NDCG)
%are both metrics designed to score search engine results by taking rank
%order into account~\cite{ndcg-sigir00}. Yilmaz \etal~\cite{new_rank-sigir08} and
%Carterette~\cite{rank_correlation-sigir09} both propose new probabalistic metrics that
%penalize errors at low ranks without requiring explicit rank weights.
%Sculley~\cite{sculley-siam07} and Kumar \etal~\cite{general_dist-www10}
%extend Kendall's $\tau$ by taking item similarity into account.

%Unfortunately, these metrics are not suitable for
%use in our study. The above metrics are designed to streamline the comparison of ranked lists
%down to a single value that is suitable for evaluating and optimizing IR systems.
%In our work, we aim for a more nuanced understanding of the differences between lists
%of search results, \ie we want to examine overlap and position switching separately.
%Sun \etal propose a method for visualizing different results from search engines that
%is based on expected weighted Hoeffding distance~\cite{sun-2010-visualizing}. Although this
%technique is very promising, it does not scale to the size of our experiments.

\paragraph{Comparing Search Engines} Several studies have examined the differences between
results from different search engines. Two studies have performed user studies to compare
search engines~\cite{vaughan-2004-measurements,barilan-2007-rankings}.
Although both studies uncover significant differences between competing search engines,
neither study examines the impact of personalization. Sun \etal propose a method for
visualizing different results from search engines that is based on expected weighted
Hoeffding distance~\cite{sun-2010-visualizing}. Although this
technique is very promising, it does not scale to the size of our experiments.

%\paragraph{Learning to Rank} A large amount of research has been conducted on using implicit
%user information to improve the ranking of search engines. Studies have examined clickthrough
%of search results~\cite{radlinski-2005-clicks,joachims-2005-clickthrough,radlinski-2007-clickthrough,dupret-2008-clicks,chapelle-2009-clicks,hu-2011-clicks},
%dwell time on webpages~\cite{agichtein-2006-dwell}, and even cursor
%tracking~\cite{guo-2012-dwell} as signals to solve the learning to rank problem.
%However, these studies are focused on improving the overall quality of the search index,
%not leveraging user information to personalize search results.

% more personalized search cites: jeh-2003-scaling

\paragraph{Personalization} Personalized search has been extensively studied in the
literature~\cite{pretschner-1999-personalize,liu-2002-categories,pitkow-2002-personalized,shen-2005-modeling,teevan-2005-personalized,sun-2005-personalized,qiu-2006-personalized,tan-2006-personalized}.
Dou~\etal provide a comprehensive overview of techniques for personalizing
search~\cite{dou-2007-personalized}.
They evaluate many strategies for personalizing search, and conclude that mining user click
histories leads to the most accurate results. In contrast, user profiles have low utility.
The authors also note that personalization is not useful for all types of queries.
\newtext{A recent study is investigating the inherent biases of search engines and 
their impact on the quality of information that reaches people.~\cite{white-2013-websearchbias} 
They show that the combined effect of people's preferences and the system's inherent bias results 
in settling on incorrect beliefs about half of the time.} 

Other features besides click history have been used to power personalized search. Three
studies leverage geographic location to personalize search~\cite{andrade-2006-relevance,yu-2007-geographic,yi-2009-geointention}. Two studies have shown that user demographics can be reliably
inferred from browsing histories, which can be useful for personalizing
content~\cite{hu-2007-predicting,goel-2012-icwsm}. To our knowledge, only one study has
investigated privacy-preserving personalized search~\cite{xu-2007-private}. Given growing
concerns about the Filter Bubble effects, this area seems promising for future research.

Several studies have looked at personalization on systems other than search. Two studies have
examined personalization of targeted ads on the Web~\cite{guha-2010-ads,wills-2012-ads}.
One study examines discriminatory pricing on e-commerce sites, which is essentially
personalization of prices~\cite{mikians-2012-prices}.

In contrast to prior research which focused on building personalized Web services, work is
now emerging that has similar goals to this study, \ie quantifying personalization on
deployed Web services. Majumder \etal propose a latent variable
model to infer the features that a service provider is using to personalize content for
a given user~\cite{majumder-2013-personalization}.







